Contextualized Spatio-Temporal Contrastive Learning with Self-Supervision

Modern self-supervised learning algorithms typically enforce persistency of instance representations across views. While being very effective on learning holistic image and video representations, such an objective becomes sub-optimal for learning spatio-temporally fine-grained features in videos, where scenes and instances evolve through space and time. In this paper, we present Contextualized Spatio-Temporal Contrastive Learning (ConST-CL) to effectively learn spatio-temporally fine-grained video representations via self-supervision. We first design a region-based pretext task which requires the model to transform in-stance representations from one view to another, guided by context features. Further, we introduce a simple network design that successfully reconciles the simultaneous learning process of both holistic and local representations. We evaluate our learned representations on a variety of downstream tasks and show that ConST-CL achieves competitive results on 6 datasets, including Kinetics, UCF, HMDB, AVA-Kinetics, AVA and OTB.

==> ConST-CL (Arxiv-2)/1.Introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% SSL, image->video SSL.
% Self-supervised learning(SSL) paves an avenue to achieve the next level of machine intelligence.
Self-supervised learning (SSL) has revolutionized natural language processing~\cite{lan2020albert, devlin2018bert} and computer vision~\cite{chen2020simclr, grill2020byol, akbari2021vatt, alayrac2020mmv} due to strong representations learned from a vast amount of unlabeled data.
% Self-supervised learning (SSL) has been shown to either achieve state-of-the-art results in many vision applications or facilitate downstream tasks with effective models that can be fine-tuned for significant performance gains. 
% On image tasks, various self-supervised learning frameworks were proposed. 
The key breakthroughs that paved the way for SSL's success in computer vision come from the instance discrimination pretext task~\cite{dosovitskiy2014discriminative} and the contrastive objective~\cite{oord2018info_nce}, with which for the first time the self-supervised pretraining surpasses the supervised pretraining on downstream visual tasks~\cite{he2019moco}.
% Self-supervised learning methods learn effective representations by exploiting instance discrimination to solve pretext tasks~\cite{dosovitskiy2014discriminative}.
%
% With the contrastive predictive coding scheme~\cite{oord2018info_nce}, self-supervised training methods have been shown to outperform supervised training approaches on many vision, audio, and natural language processing applications. 
%
% The representative frameworks for self-supervised learning on images include MoCo~\cite{he2019moco}, SimCLR~\cite{chen2020simclr}, BYOL~\cite{grill2020byol} and SwAV~\cite{caron2020swav}.
% In video domain, the annotation cost is dramatically increased for curating high-quality labeled dataset.
% And it's reportedly less publicly available video datasets~\cite{}\lzyuan{Not clear if the claim is precise here.}, especially on dense video tasks like object detection, semantic segmentation\lzyuan{Maybe not segmentation, as I can think of KITTI, Cityscapes etc.}.
% Thus adopting self-supervision in videos would be a natural choice.
% There are many works~\cite{qian2021cvrl, feichtenhofer2021rho_moco, lee2017sorting, akbari2021vatt, alayrac2020mmv} that leverage spatial, temporal or multi-modality clues emerged in videos for self-supervision showing exciting results on video understanding. 
% Examples of those works include ~\cite{} which predicts into the future, ~\cite{} which predicts temporal orders, ~\cite{} which learns from different modalities and more.
% Most recently, ~\cite{qian2021cvrl} proposed a spatio-temporally consistent data augmentation and achieved strong results on action recognition tasks by applying contrastive learning objectives.
% ~\cite{feichtenhofer2021rho_moco} further conducted a large-scale study on self-supervised video representation learning.
% \lzyuan{(MH: the transition from previous sentence to this one is not smooth.) Is current form better?}
For videos, many self-supervised contrastive learning approaches~\cite{qian2021cvrl,feichtenhofer2021rho_moco, akbari2021vatt, alayrac2020mmv} directly extend established image-based methods~\cite{he2019moco,chen2020simclr} to the spatio-temporal domain. 
Most of them, however, do not explicitly exploit the temporal evolutions of multiple instances and scene context in videos.

Self-supervised learning methods typically enforce semantic consistency across views to construct instance representations~\cite{he2019moco, chen2020simclr}. 
%
%MH: check this sentence. 
This assumption is particularly true in the image domain because two views are typically generated from the same image.
As shown in Fig.~\ref{fig:task_a}, the goal is to enforce the representations of these two views to be as close as possible in the feature space.
%
In the video domain, these view-based contrastive approaches~\cite{qian2021cvrl, feichtenhofer2021rho_moco} may be less effective as the visual appearance of an instance frequently and drastically changes across frames. 
%
For example, one person in a video can have different poses and perform different activities over time, indicating the states and semantics of an instance are likely to change across space and time.
%
Enforcing spatio-temporal persistency throughout the video~\cite{feichtenhofer2021rho_moco} would lead to representations only encoding minimally shared information across frames, which may negatively impact spatio-temporally fine-grained downstream tasks.
% \lzyuan{Need to link the motivation to the downstream tasks that we studied.}
% In this case, we are motivated to rethink the instance discrimination and redesign it for the video self-supervised learning.
% The desire of relaxing the spatio-temporal persistency and learning semantically persistent but discriminative representations is more eager for some fine-grained spatio-temporal video tasks, for example video action recognition and tracking.  
% Image/Video difference and ignorance.

% Fine-grained features learning in SSL.
Furthermore, existing self-supervised methods typically focus on learning representations for holistic visual understanding tasks~\cite{chen2020simclr, qian2021cvrl}, such as image classification and video action recognition.
% Aforementioned works are designed to learn to produce one representation per image or video, which will be evaluated on tasks such as image classification or video action recognition.
For dense prediction tasks, such as object detection, action localization and tracking, those models are enhanced by adding task specific heads.
% Recent studies~\cite{xie2021detco, yang2021inst_loc} show, however, such modification is a sub-optimal solution as during the pre-training stage the model doesn't maintain discriminative local features, which on the other hand could be beneficial for the dense visual understanding.
% Several works are dedicated to learn discriminative local features for the dense prediction tasks, for instance DenseCL~\cite{wang2021densecl} and InstLoc~\cite{yang2021inst_loc} on images, and VINCE~\cite{gordon2020vince} and VFS~\cite{xu2021vfs} on videos.
On the other hand, several approaches are designed to learn discriminative local features for dense prediction tasks~\cite{wang2021densecl, yang2021inst_loc, gordon2020vince, xu2021vfs},
%
% One limitation of those schemes is while they show superior performance on dense tasks, 
% the model's holistic visual understanding  is deficient~\cite{xie2021detco}.
but their performances on holistic visual understandings are often compromised~\cite{xie2021detco}.
% A clear phenomenon appeared on those schemes is when better performance is achieved on dense tasks, the performance on tasks that requires holistic understanding deficient~\cite{xie2021detco}.
%
% \lzyuan{Maybe need to add a statement of we want to achieve co-training and why.}
%
In light of this, we are interested in learning representations that can be applied to both holistic and local video tasks.
%as the long-standing knowledge of hierarchy~\cite{} in computer vision suggests the local and global features could bootstrap each other.
%
% DetCo~\cite{xie2021detco} tried to address the issue in image domain by enforcing consistency between global image and local patches simultaneously.

% Method and Results overviews
We propose Contextualized Spatio-Temporal Contrastive Learning (\ours), illustrated in Fig.~\ref{fig:task_b},
% to relax the strong spatio-temporal persistency across the entire video,
to circumvent the undesirable strong spatio-temporal persistency enforced by the global contrastive objective.
%to enforce the spatio-temporal persistency across the whole video,
\ours learns semantically consistent but discriminative local representations for various video downstream tasks, 
% such as spatio-temporal action localization, object tracking, etc., in addition to the traditional holistic video understanding tasks, such as video action recognition.
ranging from spatio-temporal action localization and object tracking to action recognition.
% Our insight is the same instance appeared in different context could have slightly different semantic meaning.
Specifically, 
% instead of projecting representations into one shared feature space, 
we design a projection function $g(\cdot, \cdot)$ to take not only the instance feature but also the context feature into account,
%
where the instance feature is extracted from the source view of a video, and the context feature is sampled from the target view.
% , and the function $g(\cdot, \cdot)$ transforms the instance representation $h$ from the source view into the target view conditioned on the context.
%
% By design, the context features $F_c^\prime$ guide the transformation of $h$, and the loss objective encourages similarity between the transformed representation and its corresponding representation observed in the target view.
%
This task enforces the model 
% to learn the structure of the event and 
to be context-aware in a video and thus is a good proxy to learn discriminative local representations.
% This task enforces the model to learn discriminative local representations in a video while being aware of video context and structures.
%

To address the imbalanced capability of learning holistic and local video representations, we design a simple two-branch module to facilitate the network to learn high-quality video representations both globally and locally in one unified self-supervised learning scheme.
% To resolve the in-balanced capability of simultaneous learning holistic and local representation learning, we propose a simple yet effective modification to our network architecture to learn holistic and local representations under a single learning scheme that both achieve state-the-of-the-art performances.

% We evaluate the proposed method on two tasks to analyze the quality of the spatio-temporal representations: instance-level 
% action localization on the AVA-Kinetics~\cite{li2020avak} dataset and object tracking on the OTB2015~\cite{wu2013otb}  benchmark.
% %
% For action recognition on benchmark datasets, e.g., Kinetics400~\cite{kay2017k400}, UCF101~\cite{soomro2012ucf101} and HMDB51~\cite{kuehne2011hmdb}, it entails holistic visual understanding.
%
We evaluate the learned representations on a variety of downstream tasks.
For holistic representations, we evaluate with video action recognition on Kinetics400~\cite{kay2017k400}, UCF101~\cite{soomro2012ucf101} and HMDB51~\cite{kuehne2011hmdb} datasets. 
For local representations, we conduct experiments with spatio-temporal action localization on AVA-Kinetics~\cite{li2020avak} and AVA~\cite{gu2018ava} datasets, and the single object tracking on the OTB2015~\cite{wu2013otb} dataset.
%
Our experimental results show that by pretraining with \ours, the learned representations 
adapt well across all studied datasets, surpassing recently proposed methods that use either supervised pretraining or the self-supervised pretraing~\cite{qian2021cvrl, xu2021vfs, feichtenhofer2021rho_moco, girdhar2019vat}.
%
% On all these tasks and datasets, \ours outperforms almost all the baselines~\cite{qian2021cvrl,xu2021vfs,feichtenhofer2021rho_moco}.

% Contributions
The main contributions of this work are:
%\begin{itemize}
\begin{compactitem}
    \item A region-based contrastive learning framework for fine-grained spatio-temporal representation learning.
    \item A contextualized region prediction task that facilitates learning semantically consistent while locally discrinimative video features.
    % \item We unify the holistic and local representation learning with self-supervision in video by designing a network architecture.
    \item A simple network design to effectively reconcile simultaneous holistic and local representation learning.
    \item Competitive performance on 6 benchmarks, including spatio-temporal action localization, object tracking, and video action recognition.  
    %
    %On AVA-Kinetics~\cite{li2020avak}, \ours achieves 38.1$\%$ mAP and 28.8$\%$ mAP using ground-truth and detected boxes respectively;
    %On OTB2015~\cite{wu2013otb}, \ours achieves 78.8 precision and 54.3 success score;
    %On video-level action recognition tasks, \ours achieves 94.9$\%$ and 69.4$\%$ Top-1 accuracy on UCF101~\cite{soomro2012ucf101} and HMDB51~\cite{kuehne2011hmdb}.
    %MH: no need to brag too much
    %, building up the new records of these benchmark with self-supervised learning.
    
%\end{itemize}
\end{compactitem}

==> ConST-CL (Arxiv-2)/2.RelatedWork.tex <==
\section{Related Work}
\label{sec:related_work}
% Self-supervised learning is an attracting domain to study as it alleviates the requirement of expensive human-annotated dataset and enables to leverage the large amount of unlabeled data in the wild.

\noindent \textbf{Self-supervised learning in images.}
% \noindent \textbf{Image reprensetation SSL.} 
To effectively learn representations from images, early self-supervised methods focus on designing pretext tasks by experts.
%
Various pretext tasks have been proposed, including colorization~\cite{larsson2017colorization}, inpainting~\cite{pathak2016context}, denoising~\cite{vincent2008extracting}, egomotion prediction~\cite{agrawal2015learning}, context prediction~\cite{doersch2015unsupervised}, orientation prediction~\cite{gidaris2018rotations}, spatial jigsaw puzzle~\cite{noroozi2016jigsaw}, \etc. 
%
Recent advances in image self-supervised learning stem mainly from minimizing contrastive loss~\cite{oord2018info_nce} on instance discrimination tasks~\cite{dosovitskiy2014discriminative}.
%
The contrastive objective effectively enforces representations of the same instance from different views to be similar, while it repels representations from different instances in the latent space. 
%
Representative frameworks in this category include NPID~\cite{wu2018npid}, MoCo~\cite{he2019moco, chen2020moco_v2}, SimCLR~\cite{chen2020simclr}, \etc.

\vspace{1mm}
\noindent \textbf{Self-supervised learning in videos.} 
% \noindent \textbf{Video reprensetation SSL.} 
In the video domain, self-supervised representation learning prospers in recent years.
%
%The reasons behind this are first, the cost of curating a high-quality large-scale video dataset is high, which poses the self-supervised learning an appealing position.
%
%Second, videos by nature host more signals that are easy to exploit for self-supervised learning.
Contrastive objectives have been widely used to learn video representations for holistic recognition tasks~\cite{qian2021cvrl, feichtenhofer2021rho_moco, recasens2021brave, yang2020tempo, singh2021semi}.
% pretext tasks 
Extensive pretext tasks have been exploited to learn good representation in videos. 
%
Compared with the image domain, videos naturally yield richer self-supervision signals. 
% views, context.
In~\cite{recasens2021brave}, the goal is to enforce global context consistency and utilize long-short views of a video to align representations.
%
In~\cite{wang2018pulling}, the action and context features are factorized separately by learning from the conjugate examples in video dataset.
% motion, optical flow
Motion signals are also exploited for learning good representations~\cite{tian2020contrastive, han2020self-motion}.
% temporal/future prediction
Temporal ordering of frames in a video has also been used for self-supervised representation learning.
% ~\cite{} predicts into the future.
%
For instance, in~\cite{misra2016shuffle, lee2017sorting}, temporal ordering of frames is enforced to learn representations by scuffling frames in a self-supervised manner.  
%
Similarly, forward and backward ordering of frames is used as the self-supervision signals for representation learning~\cite{wei2018arrow}.
%
In addition, temporal cycle consistency is exploited to learn spatio-temporal correspondence between video frames~\cite{jabri2020random_walk,wang2019cycle}.
% multi-modal
On the other hand, multi-modal signals, such as audio/visual and visual/text, have been used to learn representations in a self-supervised manner that outperform models based on a single modality~\cite{alayrac2020mmv, alwassel2019self, patrick2021compositions, morgado2020audio}.  

% \textbf{Learning local features with self-supervision.} 
\vspace{1mm}
\noindent \textbf{Local representations.} 
Although existing methods focus on learning holistic representations on images or videos, several recent approaches explicitly model spatially fine-grained representations.
%
In~\cite{chaitanya2020contrastive_global_local, wang2021densecl},
several constriave learning models have been developed for dense prediction tasks, such as object detection and image segmentation.
%
In addition, augmented samples with 
pseudo ground-truth are generated to learn dense features for object detection~\cite{yang2021inst_loc, ding2021patch_reid}.
%
Other methods introduce location priors to group pixels for learning local features. For example,~\cite{zhang2020self_xiao, henaff2021cont_det, van2021unsupervised_van_gool} use unsupervised masks and~\cite{pinheiro2020vader, xie2021propagate} use pixel coordinates.
%
In the video domain, 
many methods learn fine-grained features by leveraging inherent temporal augmentations to determine object correspondence~\cite{xu2021vfs, yao2020seco, gordon2020vince, jabri2020random_walk}.
% 
\cite{gordon2020vince} randomly samples two images from a video to construct the contrastive pairs for self-supervised learning and shows improved performance on video tasks.
\cite{yao2020seco} employs pretext tasks of determining whether frames are from the same video and their temporal ordering.
\cite{xu2021vfs} observes the emergence of correspondence by learning frame-level similarity.
\cite{jabri2020random_walk} enforces forward-backward temporal consistency to learn local correspondences in videos.
%
%Most of these methods, however, focus thinly on the  local  representation  learning  and  the  performance  on image/video-level recognition tasks are deficient.
Most of the existing approaches focus on learning local representations and do not emphasize performances on holistic tasks. \cite{xie2021detco} explicitly raises the question about simultaneously learning holistic and local representations but only focuses on the image domain.

Different from these related works, our method leverages video context during self-supervised learning by employing a novel region-based prediction tasks, and is designed to learn holistic and local representations simultaneously with self-supervision from unlabeled videos. 
Unlike most of the aforementioned methods that focus on learning either holistic or local representations, we emphasize the quality of both under one unified training scheme.

==> ConST-CL (Arxiv-2)/3.Method.tex <==
\section{Method}
\label{sec:method}

In this section, we introduce the proposed self-supervised learning framework, Contextualized Spatio-Temporal Contrastive Learning (\ours) for learning spatio-temporally fine-grained representations in videos.
% %
% % Building on the spatio-temporal contrastive video representation learning framework~\cite{qian2021cvrl}, we propose to simultaneously learn both holistic and local video representations simultaneously.
% % % We adopt the same data augmentation protocol and the model architecture when possible and careful design the learning procedures.
% % With moderate computational overhead than the baseline~\cite{qian2021cvrl}, we show that the learned representations can be generalized well to both clip-level and instance-level downstream tasks, including action recognition, action localization and single object tracking.
% % Under the contrastive video representation learning paradigm~\cite{qian2021cvrl}, we first describe a vanilla self-supervised framework for simultaneously learning holistic and local video representations.
% % In this section, we first describe a vanilla region-based contrastive learning method in extension of~\cite{qian2021cvrl, wang2021densecl} for learning local video representations.
% We first describe a vanilla region-based contrastive learning method as an extension of~\cite{qian2021cvrl, wang2021densecl}. % for learning local video representations.
% Then, we describe \ours in details which improves local video representation learning.
% Finally, we discuss how to generate region priors and to effectively balance global and local learning.

\input{Tex/Method/1.instance_constrastive_learning}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/global_local_losses_v5.pdf}
    \vspace{-15pt}
    \caption{
    \textbf{Balancing global and local losses.}
    We analyze three different endpoints to impose global and local training losses. 
    $\otimes$ indicates a pooling operation.
    %
    Throughout the experiments, we find that by branching the res5 block in the network and applying $\mathcal{L}_g$ and $\mathcal{L}_r$ on R$5_g$ and R$5_r$ respectively, two losses mutually benefit and the representations thrive by co-training.
    }
    \label{fig:global_local_loss}
    \vspace{-5pt}
\end{figure}

\input{Tex/Method/2.contextualized_instance_prediction}
\input{Tex/Method/3.instance_locations.tex}

\input{Tables/main_table.tex}

\input{Tex/Method/4.balance_global_local.tex}

==> ConST-CL (Arxiv-2)/4.Experiments.tex <==
\section{Experiments}
\label{sec:experiments}

% We evaluate the proposed method on various downstream tasks. 
%
We evaluate clip-level video representation models on the Kinetics400~\cite{kay2017k400} dataset following the linear probing protocol, and the UCF101~\cite{soomro2012ucf101} and  HMDB51~\cite{kuehne2011hmdb} datasets using both linear probing and fine-tuning.
%
To evaluate the learned spatio-temporally fine-grained representations, we conduct experiments on the  AVA-Kinetics~\cite{li2020avak} and AVA v2.2~\cite{gu2018ava} datasets for spatio-temporal action localization and the OTB2015~\cite{wu2013otb} dataset for single object tracking.

\input{Tex/Experiments/1.experiment_setup.tex}
\input{Tex/Experiments/2.downstream_evaluations}
\input{Tex/Experiments/3.main_results.tex}
\input{Tables/video_classification.tex}
\input{Tables/model_size.tex}

\input{Tables/temporal_sampling.tex}
\input{Tables/endpoints.tex}

\input{Tables/context_length_and_overhead.tex}
\input{Tables/box_type.tex}
\input{Tex/Experiments/4.ablation_studies}

\subsection{Limitations}
% In our experiments, we show that \ours achieves great performance on holistic and instance-level video understanding tasks. % such as spatio-temporal action localization and object tracking.
% We are also interested in learning the denser spatio-temporal representations which could be potentially beneficial to the even finer-grained video task.
One missing piece in the current framework is the self-supervisory signal for learning even finer-grained representations.
% We hope to enrich our method by incorporating dense self-supervision and conduct experiments on dense video tasks such as video object segmentation in the future. 
We hope to enrich our method by incorporating dense self-supervision in the future. 
Moreover, the current solution of organizing global-local self-supervisory signals is limited to the convolutional neural network backbone.
For the recent vision transformer (ViT)~\cite{dosovitskiy2020vit}, it is non-trivial to apply our proposed method directly in its current form. 
% We are interested in exploring solutions that benefit ViT-like architectures with self-supervision.

==> ConST-CL (Arxiv-2)/5.Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

%MH: I usually put limitation as one paragraph or ssection in Experiments. 
% \lzyuan{Limitations}

%MH: check all sentences in text/tables/figures and use current tense 
In this paper, we propose a novel self-supervised learning framework that facilitates learning versatile spatio-temporally fine-grained representations in videos. 
%
A simple architecture design is proposed to reconcile holistic and local representations learning in one single framework.
%
Extensive experiments are carried out to demonstrate the efficacy of the proposed method.  
%
%We hope this method could inspire more research on the self-supervised learning.
%
In the future, we plan to experiment on more video tasks, such as video segmentation and temporal localization.
%
%Ultimately, we hope to develop an unified self-supervised learning framework that learns hierarchical representations and solve different level of video understanding tasks. 

\noindent \textbf{Acknowledgment.} We thank Olivier Henaff (DeepMind) for providng image segmentation code; Ang Li (DeepMind) for the help with AVA-Kinetics; Xiao Zhang (U. Chicago) and Jianing Wei (Google) for the help with object tracking.

==> ConST-CL (Arxiv-2)/Sup_Materials/attention.tex <==
\begin{figure*}[t!]
\centering
% \scriptsize
\setlength\tabcolsep{1pt} % default value: 6pt
\begin{tabular}{cccc}
  Source &
  Thumbnail & 
  Target &
  Attention
\\
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000036_v4_source.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000036_v4_source_thumbnail.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000036_v4_target.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000036_v4_att.jpeg}} 
 \\ 
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000001_v4_source.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000001_v4_source_thumbnail.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000001_v4_target.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000001_v4_att.jpeg}} 
 \\ 
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000033_v4_source.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000033_v4_source_thumbnail.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000033_v4_target.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000033_v4_att.jpeg}} 
 \\ 
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000022_v4_source.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000022_v4_source_thumbnail.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000022_v4_target.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000022_v4_att.jpeg}} 
 \\ 
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000025_v4_source.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000025_v4_source_thumbnail.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000025_v4_target.jpeg}} &
 {\includegraphics[width=0.23\linewidth]{Sup_Materials/Figures_resized/video_000025_v4_att.jpeg}} 
 
  \end{tabular}
  \centering
  \caption{
  \textbf{Visualization of the attention during the training.}
  We use boxes from the object detector to pool region features from the source view as the query in order to generate the attention maps given the context (features from the target view).
  Interestingly, the model learns to attend to not only the corresponding instance in the target frame, but also to some other semantically meaningful objects the instance potentially interacts with.
  }
  \vspace{-15pt}
  \label{fig:attention}
\end{figure*}

==> ConST-CL (Arxiv-2)/Sup_Materials/r3d_table.tex <==
% \newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1pt}}
\newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth\global\arrayrulewidth 1pt}\hline\noalign{\global\arrayrulewidth\savewidth}}
% 
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}
% 
\newcommand{\blocks}[3]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{1$\times$1$^\text{2}$, #2}\\[-.1em] \text{1$\times$3$^\text{2}$, #2}\\[-.1em] \text{1$\times$1$^\text{2}$, #1}\end{array}\right]\)$\times$#3}}
% 
\newcommand{\blockt}[3]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{\underline{3$\times$1$^\text{2}$}, #2}\\[-.1em] \text{1$\times$3$^\text{2}$, #2}\\[-.1em] \text{1$\times$1$^\text{2}$, #1}\end{array}\right]\)$\times$#3}}


\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{
        \tablestyle{5pt}{1.1}
        \begin{tabular}{c|c|c|c}
            \shline
            Stage & Network & Input from & Output size $T \times S^2$ \\
            \shline
            raw clip & - & - & $32\times224^\text{2}$ \\
            \hline
            data & stride \textbf{2}, 1$^\text{2}$ & raw clip & $16\times224^\text{2}$ \\
            \hline
            \multirow{2}{*}{res1} &
            \multicolumn{1}{c|}{\underline{$\textbf{5}\times7^\text{2}$}, {64}} &
            \multirow{2}{*}{data} &
            \multirow{2}{*}{$8\times112^\text{2}$}  \\
            & stride \textbf{2}, 2$^\text{2}$ & \\
            \hline
            \multirow{2}{*}{pool1} &
            \multicolumn{1}{c|}{$1\times3^\text{2}$ max} & 
            \multirow{2}{*}{res1} &
            \multirow{2}{*}{$8\times56^\text{2}$} \\
            & stride 1, 2$^\text{2}$ & \\
            \hline
            \multirow{3}{*}{res2} & \blocks{{256}}{{64}}{3} &
            \multirow{3}{*}{pool1} &
            \multirow{3}{*}{$8\times56^\text{2}$}  \\
            &  & \\
            &  & \\
            \hline
            \multirow{3}{*}{res3} & \blocks{{512}}{{128}}{4} &
            \multirow{3}{*}{res2} & 
            \multirow{3}{*}{$8\times28^\text{2}$}  \\
            &  & \\
            &  & \\
            \hline
            \multirow{3}{*}{res4} & \blockt{{1024}}{{256}}{6} & 
            \multirow{2}{*}{res3} &
            \multirow{3}{*}{$8\times14^\text{2}$} \\
            &  & \\
            &  & \\
            \hline
            \multirow{3}{*}{res5$_{r}$} & \blockt{{2048}}{{512}}{3} &
            \multirow{2}{*}{res4} &
            \multirow{3}{*}{$8\times7^\text{2}$} \\
            &  & \\
            &  & \\
            \hline
            \multirow{3}{*}{res5$_g$} & \blockt{{2048}}{{512}}{3} &
            \multirow{2}{*}{res4} &
            \multirow{3}{*}{$8\times7^\text{2}$} \\
            &  & \\
            &  & \\
            % \hline
% 			\multicolumn{2}{c|}{global average pooling} &  $1\times1^\text{2}$ \\
			\shline
    \end{tabular}
    }
    \vspace{2mm}
    \caption{\textbf{Base network $\boldsymbol{f(\cdot)}$: a ResNet3D-50 (R3D-50) based encoder.} 
    % The input video has 16 frames (stride 2) in self-supervised pre-training.
    % and 32 frames (stride 2) in linear evaluation, semi-supervised learning, supervised learning and downstream tasks.
    }
    \label{tab:r3d_network}
\vspace{-4mm}
\end{table}

==> ConST-CL (Arxiv-2)/Sup_Materials/tracker.tex <==
\begin{figure*}[t!]
\centering
% \scriptsize
\setlength\tabcolsep{1pt} % default value: 6pt
\begin{tabular}{c|ccccc}
  Input & \multicolumn{5}{c}{Prediction}
\\
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/BlurCar1_000000.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/BlurCar1_000010.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/BlurCar1_000020.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/BlurCar1_000030.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/BlurCar1_000040.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/BlurCar1_000050.jpeg}} \\
 
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/DragonBaby_000000.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/DragonBaby_000010.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/DragonBaby_000020.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/DragonBaby_000030.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/DragonBaby_000040.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/DragonBaby_000050.jpeg}} \\
 
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Tiger1_000000.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Tiger1_000010.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Tiger1_000020.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Tiger1_000030.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Tiger1_000040.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Tiger1_000050.jpeg}} \\
 
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Soccer_000000.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Soccer_000010.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Soccer_000020.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Soccer_000030.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Soccer_000040.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Soccer_000050.jpeg}} \\
 
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Skiing_000000.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Skiing_000010.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Skiing_000020.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Skiing_000030.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Skiing_000040.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Skiing_000050.jpeg}} \\
  
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Couple_000000.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Couple_000010.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Couple_000020.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Couple_000030.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Couple_000040.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Couple_000050.jpeg}} \\
 
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Surfer_000000.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Surfer_000010.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Surfer_000020.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Surfer_000030.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Surfer_000040.jpeg}} &
 {\includegraphics[width=0.16\linewidth]{Sup_Materials/Figures_resized/tracker/Surfer_000050.jpeg}} \\
 
  \end{tabular}
  \centering
  \caption{ 
  Qualitative results for visual object tracking on OTB2015~\cite{wu2013otb}. Best view in color.
  }
%   \vspace{-15pt}
  \label{fig:tracker}
\end{figure*}

==> ConST-CL (Arxiv-2)/Sup_Materials/tx_table.tex <==
% \newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth\global\arrayrulewidth 1pt}\hline\noalign{\global\arrayrulewidth\savewidth}}
% % 
% \newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}
% % 
% \newcommand{\blocks}[3]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{1$\times$1$^\text{2}$, #2}\\[-.1em] \text{1$\times$3$^\text{2}$, #2}\\[-.1em] \text{1$\times$1$^\text{2}$, #1}\end{array}\right]\)$\times$#3}}
% % 
% \newcommand{\blockt}[3]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{\underline{3$\times$1$^\text{2}$}, #2}\\[-.1em] \text{1$\times$3$^\text{2}$, #2}\\[-.1em] \text{1$\times$1$^\text{2}$, #1}\end{array}\right]\)$\times$#3}}

\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
        \tablestyle{5pt}{1.1}
        \begin{tabular}{c|c|c|c}
            \shline
            Stage & Input, Dimension & Network & Output \\
            \shline
            Linear project & $\boldsymbol{h}$, N$\times$2048 & n\_nodes=128 & Query \\
            \hline
            Linear project & $\boldsymbol{F_c^\prime}$, M$\times$2048 & n\_nodes=128 &  Key \\
            \hline
            Linear project & $\boldsymbol{F_c^\prime}$, M$\times$2048 & n\_nodes=128 &  Value \\
            \hline
            \multirow{3}{*}{MHSA} & Query, N$\times$128 & hidden\_size=128 & \multirow{3}{*}{Hidden} \\
            & Key, M$\times$128 & n\_heads=3 & \\
            & Value, M$\times$128 & n\_layers=3 & \\
            % & & \\
            \hline
            Linear project & Hidden, N$\times$128 & n\_nodes=2048 & $\boldsymbol{z}$ \\
			\shline
    \end{tabular}
    }
    \vspace{2mm}
    \caption{\textbf{\ours head $\boldsymbol{g(\cdot, \cdot)}$: a transformer-based decoder.} 
    The inputs are the region features $\boldsymbol{h}$ and the context features $\boldsymbol{F_c^\prime}$ and the outputs are the transformed features $\boldsymbol{z}$. N and M are the number of tokens of $\boldsymbol{h}$ and $\boldsymbol{F_c^\prime}$ respectively.}
    \label{tab:tx_network}
\vspace{-4mm}
\end{table}

==> ConST-CL (Arxiv-2)/Tables/box_type.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{cccccc} 

\hline
 & UCF & AVA-K & \multicolumn{2}{c}{OTB} \\
\cline{4-5}
Box type & Top-1 & mAP (GT) & Precision & Success \\
\hline
Random & $94.3$ & $36.9$ & $77.0$ & $54.0$ \\
SLIC~\cite{achanta2012slic} & $93.4$ & $36.4$ & $76.3$ & $53.7$ \\
FH~\cite{felzenszwalb2004fh_seg} & $94.1$ & $36.9$ & $77.1$ & $54.3$ \\
Person Detector & $93.4$ & $36.7$ & $77.7$ & $55.0$ \\
Object Detector & $93.7$ & $37.2$ & $77.8$ & $54.1$ \\
\hline

\end{tabular}
% \vspace{-5pt}
\caption{
\textbf{Ablation study on the box type.}
When applying different types of boxes during the self-supervised training, 
we find that model learns equally well regardless of the region location quality.}
\label{tab:box_type}
\vspace{-5pt}
\end{table}

==> ConST-CL (Arxiv-2)/Tables/computational_cost.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{cccc} 

\hline
Context length & Endpoint & $\#$ Params (M) & FLOPs (B) \\
\hline
- & - & $44.60$ & $45.58$ \\
% $0$ & R5 & $57.48$ & $45.68$ \\
$0$ & 2R5 & $77.71$ & $55.45$ \\
$1$ & 2R5 & $71.76$ & $55.60$ \\
% $3$ & 2R5 & $71.76$ & $56.07$ \\
$5$ & 2R5 & $71.76$ & $56.53$ \\
\hline

\end{tabular}
\caption{
Ablation study on the computational cost. 
We notice the number of parameter increment is largely from the duplicated $res5$ block while our transformer based head is more parameter efficient than the MLP head for the region-based contrastive learning.
}
\label{tab:cost}
\end{table}

==> ConST-CL (Arxiv-2)/Tables/context_length.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{cccccc} 

\hline
Context &  \multicolumn{2}{c}{AVA-Kinetics} & &  \multicolumn{2}{c}{OTB}\\
\cline{2-3} \cline{5-6}
length & mAP (GT) & mAP (Det) & & Precision & Success\\
\hline
 - & $30.9$ & $23.4$ & & $75.9$ & $53.6$ \\
$0$ & $35.3$ & $27.5$ & & $75.4$ & $56.6$ \\
$1$ & $36.7$ & $28.0$ & & $77.7$ & $55.0$ \\
$3$ & $36.9$ & $28.1$ & & $77.5$ & $54.5$ \\
$5$ & $37.6$ & $28.1$ & & $79.0$ & $55.4$ \\
\hline

\end{tabular}
\caption{
We analyze the effect of context length to the model performance. 
``-" indicates no \ours is used and the model is only trained with the $\mathcal{L}_g$; 
``0" indicates no context is provided and the model simply degraded to the vanilla region-based contrastive learning.
From the table, we observe the trend that more context is helpful to learn better spatio-temporal representations.}
\label{tab:context_length}
\end{table}

==> ConST-CL (Arxiv-2)/Tables/context_length_and_overhead.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{ccccccccccc} 

\hline
Context & Loss & UCF & HMDB & \multicolumn{2}{c}{AVA-Kinetics} & &  \multicolumn{2}{c}{OTB}\\
\cline{5-6} \cline{8-9}
length & endpoint(s) & Top-1 & Top-1 & mAP (GT) & mAP (Det) & & Precision & Success & $\#$Params (M) & $\#$FLOPs (G) \\
\hline
- & R5  & $91.6$ & $66.2$ & $30.9$ & $23.4$ & & $75.9$ & $53.6$ & $44.6$ & $45.6$ \\
$0$ & 2R5 & $91.8$ & $66.0$ & $35.3$ & $27.5$ & & $75.4$ & $56.6$ & $77.7$ & $55.5$ \\
$1$ & 2R5 & $93.4$ & $66.7$ & $36.7$ & $28.0$ & & $77.7$ & $55.0$ & $71.7$ & $55.6$ \\
$3$ & 2R5 & $93.7$ & $67.4$ & $36.9$ & $28.1$ & & $77.5$ & $54.5$ & $71.7$ & $56.1$ \\
$5$ & 2R5 & $93.4$ & $67.5$ & $37.6$ & $28.1$ & & $79.0$ & $55.4$ & $71.7$ & $56.5$ \\
\hline

\end{tabular}
% \vspace{-5pt}
\caption{
\textbf{Ablation study on the context length and the computational overhead.}
``-" indicates no \ours is used and the model is only trained with the $\mathcal{L}_g$; 
``0" indicates no context is provided and the model simply degrades to the vanilla region-based contrastive learning.
From the table, we observe the trend that more context is helpful to learn better spatio-temporal representations.
%
We notice the number of parameter increment is largely from the duplicated $res5$ block while our transformer based head is more parameter efficient than the MLP head for the region-based contrastive learning.
}
\vspace{-5pt}
\label{tab:context_length_and_overhead}
\end{table*}

==> ConST-CL (Arxiv-2)/Tables/endpoints.tex <==
\begin{table}[t!]
\small
\centering
\begin{tabular}{cccccc} 
\hline
 
Method & Endpoint & UCF & HMDB & AVA-K & OTB \\

\hline
CVRL & - & $91.6$ & $66.2$ & $30.9$ & $75.9$ \\
\ours & $C4_p$ & $93.5$ & $67.5$ & $32.0$ & $75.3$ \\
\ours & $C5$ & $93.4$ & $66.7$ & $33.6$ & $74.3$ \\
\ours & $C5_g$+$C5_r$ & $94.3$ & $68.7$ & $36.7$ & $77.7$ \\
\hline
\end{tabular}
\vspace{-5pt}
\caption{
\textbf{Ablation on the loss endpoints.}
We apply region-based contrastive loss on different endpoints and show that the $C5_g$+$C5_r$ configuration achieves the best trade-off between the global and local losses with the best downstream task performances.}
% \vspace{-5pt}
\label{tab:endpoints}
\end{table}

==> ConST-CL (Arxiv-2)/Tables/main_table.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{ccccccccccccccc} 
\hline
 
 &  & Pre-training & \multicolumn{2}{c}{AVA-Kinetics} & & \multicolumn{2}{c}{AVA} & & \multicolumn{2}{c}{Object Tracking} \\
\cline{4-5} \cline{7-8} \cline{10-11}
Method & Backbone & Dataset & mAP (GT) & mAP (Det) & & mAP (GT) & mAP (Det) & & Precision & Success \\

\hline
INet-sup~\cite{li2020avak} & I3D & K400 & $35.9$ & $22.9$ & & 27.5 & 19.1 & & - & -\\
% INet-sup$^{\dagger}$ & I3D & K400 & $32.0$ & $23.1$ & & - & - & & - & -\\
K400-sup & R3D50 & K400 & $26.7$ & $19.8$ & & - & 22.2 & & $71.2$ & $51.46$ \\
\hline
SimSiam~\cite{chen2021simsiam} & R50 & INet & - & - & & - & - & & $61.0$ &  $43.2$ \\
VINCE~\cite{gordon2020vince} & R50 & R2V2 & - & - & & - & - & & $66.0$ & $47.6$ \\
SeCo~\cite{yao2020seco} & R50 & K400 & - & - & & - & - & & $71.9$ &  $51.8$ \\
VFS~\cite{xu2021vfs} & R50 & K400 & - & - & & - & - & & $73.9$ &  $52.5$ \\
\hline
$\rho$MoCo~\cite{feichtenhofer2021rho_moco} & Slow-only & K400 & - & - & & - & $20.3$ & & - & - \\
$\rho$BYOL~\cite{feichtenhofer2021rho_moco} & Slow-only & K400 & - & - & & - & $23.4$ & & - & - \\
VFS-inflated & R3D50 & K400 & $34.6$ & $25.9$ & & $29.1$ & $22.4$ & &  $73.3$ & $52.7$ \\
CVRL~\cite{qian2021cvrl} & R3D50 & K400 & $31.6$ & $24.1$ & & $24.9$ & $18.4$ & & $75.4$ & $53.7$ \\
\hline
\ours & R3D50 & K400 & $\mathbf{39.4}$ & $\mathbf{30.5}$ & & $\mathbf{31.1}$ & $\mathbf{24.1}$ & & $\mathbf{78.1}$ & $\mathbf{55.2}$ & \\

\hline
\end{tabular}
\vspace{-5pt}
% \caption{We evaluate the self-supervised learning in two folds: the fine-grained spatio-temporal understanding on AVA-Kinetics and OTB and the holistic video understanding on K400, UCF101 and HMDB51.
\caption{\textbf{Downstream task performances based on pre-trained representations.} The learned representations are evaluated for spatio-temporally fine-grained tasks, including spatio-temporal action recognition on the AVA v2.2 and AVA-Kinetics (using both ground-truth and detected person boxes) and single object tracking on OTB2015.
%
\ours achieves the state-of-the-art results across the board, suggesting the effectiveness of our proposed framework that is capable of coherently learning better local visual representations in videos.}
% $^{\dagger}$ indicates our reproduced results.}
\label{tab:main_table}
\vspace{-5pt}
\end{table*}

==> ConST-CL (Arxiv-2)/Tables/main_table_bk.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{cccccccccccccccc} 
\hline
 
 &  & Pre-training & Linear & \multicolumn{2}{c}{Fine-tune} & & \multicolumn{2}{c}{Action Localization} & &  \multicolumn{2}{c}{Object Tracking} \\
\cline{5-6} \cline{8-9} \cline{11-12}
Method & Backbone & Dataset & K400 & UCF & HMDB & & AVA-K (GT) & AVA-K (Det) & & Precision & Success \\

\hline
INet-sup~\cite{li2020avak} & I3D & K400 & - & - & - & & $35.9$ & $22.9$ & & - & -\\
INet-sup$^{\dagger}$ & I3D & K400 & - & - & - & & $32.0$ & $23.1$ & & - & -\\
K400-sup & R3D50 & K400 & - & - & - & & $26.7$ & $19.8$ & & $71.2$ & $51.46$ \\
\hline
SimSiam~\cite{chen2021simsiam} & R50 & INet & - & - & - & & - & - & & $61.0$ &  $43.2$ \\
VINCE~\cite{gordon2020vince} & R50 & R2V2 & $49.1$ & - & - & & - & - & & $66.0$ & $47.6$ \\
SeCo~\cite{yao2020seco} & R50 & K400 & $61.9$ & $88.3$ & $55.6$ & & - & - & & $71.9$ &  $51.8$ \\
VFS~\cite{xu2021vfs} & R50 & K400 & - & - & - & & - & - & & $73.9$ &  $52.5$ \\
\hline
$\rho$MoCo~\cite{feichtenhofer2021rho_moco} & R3D50 & K400 & $\mathbf{67.4}$ & $93.2$ & - & & - & - & & - & - \\
VFS-inflated & R3D50 & K400 & $33.1$ & $71.4$ & $41.0$ & & $34.6$ & $25.9$ & & $73.3$ & $52.7$ \\
CVRL~\cite{qian2021cvrl} & R3D50 & K400 & $66.1$ & $92.2$ & $66.7$ & & $31.6$ & $24.1$ & & $75.4$ & $53.7$ \\
\hline
\ours & R3D50 & K400 & $66.6$ & $\mathbf{94.8}$ & $\mathbf{71.9}$ & & $\mathbf{39.4}$ & $\mathbf{30.5}$ & & $\mathbf{78.1}$ & $\mathbf{55.2}$ & \\

\hline

\end{tabular}
% \caption{We evaluate the self-supervised learning in two folds: the fine-grained spatio-temporal understanding on AVA-Kinetics and OTB and the holistic video understanding on K400, UCF101 and HMDB51.
\caption{\textbf{Downstream task performances using pre-trained representations.} The learned representations are evaluated for spatio-temporally fine-grained tasks, including spatio-temporal action recognition on AVA-Kinetics (using both ground-truth and detected person boxes) and single object tracking on OTB2015, and holistic video action recognition tasks on Kinetics400, UCF101 and HMDB51.
%
\ours achieves the state-of-the-art results across the board, suggesting the effectiveness of our proposed framework that is capable of coherently learning better holistic and local visual representations in videos.
$^{\dagger}$ indicates our reproduced results.}
\label{tab:main_table}
\vspace{-10pt}
\end{table*}

==> ConST-CL (Arxiv-2)/Tables/model_size.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{cccc} 

\hline
Method & Frames & Params (M) & FLOPs (G) \\
\hline
CVRL~\cite{qian2021cvrl} & 16$\times$2 & $44.6$ & $91.2$ \\
$\rho$MOCO ($\rho$=$2$)~\cite{feichtenhofer2021rho_moco} & 8$\times$2 & $44.6$ & $83.6$ \\
$\rho$MOCO ($\rho$=$2$)~\cite{feichtenhofer2021rho_moco} & 16$\times$2 & $44.6$ & $167.0$ \\
$\rho$BYOL ($\rho$=$4$)~\cite{feichtenhofer2021rho_moco} & 16$\times$4 & $44.6$ & $334.0$ \\
\ours & 16$\times$2 & $71.7$ & $113.0$ \\
\hline

\end{tabular}
\vspace{-5pt}
\caption{\textbf{Model sizes and computational costs} for different SSL methods with video-based networks. The SSL heads are included for the parameter and FLOPS counts.}
\label{tab:model_size}
\vspace{-5pt}
\end{table}

==> ConST-CL (Arxiv-2)/Tables/temporal_sampling.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{cccccc} 
\hline
 
%  & temporal & & & & \\
Method & Sampling & UCF & HMDB & AVA-K & OTB \\

\hline
CVRL & - & $91.6$ & $66.2$ & $30.9$ & $75.9$ \\
\ours & Random & $56.2$ & $57.8$ & $34.8$ & $75.4$ \\
\ours & Center & $94.1$ & $67.7$ & $36.9$ & $77.1$ \\
\ours & Nearest & $93.8$ & $68.1$ & $36.9$ & $76.4$ \\
\hline

\end{tabular}
\vspace{-5pt}
\caption{
\textbf{Ablation on the temporal sampling strategy.}
The ``Center" and ``Nearest" temporal sampling strategy perform equally well and better than ``Random" sampling for \ours.}
\label{tab:sampling}
\vspace{-5pt}
\end{table}

==> ConST-CL (Arxiv-2)/Tables/video_classification.tex <==
\begin{table}[t!]
\centering
\small
\setlength{\tabcolsep}{.6\tabcolsep}
\begin{tabular}{ccccccccccc} 
\hline
 & \multicolumn{3}{c}{Linear} & & \multicolumn{2}{c}{Fine-tune} \\
\cline{2-4} \cline{6-7} \cline{9-10}
Method & K400 & UCF & HMDB & & UCF & HMDB \\

\hline
% SimSiam~\cite{chen2021simsiam} & R50 & - & - & - & & - & - \\
VINCE~\cite{gordon2020vince} & $49.1$ & - & - & & - & - \\
SeCo~\cite{yao2020seco} & $61.9$ & - & - & & $88.3$ & $55.6$ & \\
\hline
VFS-inflated~\cite{xu2021vfs} & $33.1$ & - & - & & $71.4$ & $41.0$ \\
$\rho$MoCo ($\rho$=$2$)~\cite{feichtenhofer2021rho_moco} & $67.4$ & - & - & & $93.2$ & - \\
$\rho$BYOL ($\rho$=$4$)~\cite{feichtenhofer2021rho_moco} & $\mathbf{71.5}$ & - & - & & $\mathbf{95.5}$ & $\mathbf{73.6}$ \\
CVRL~\cite{qian2021cvrl} & $66.1$ & $\mathbf{89.2}$ & $57.3$ & & $92.2$ & $66.7$ \\
\hline
\ours & $66.6$ & $89.1$ & $\mathbf{59.9}$ & & $94.8$ & $71.9$ \\
\hline
\end{tabular}
% \caption{We evaluate the self-supervised learning in two folds: the fine-grained spatio-temporal understanding on AVA-Kinetics and OTB and the holistic video understanding on K400, UCF101 and HMDB51.
\caption{\textbf{Downstream video action recognition.} 
% The learned representations are evaluated on holistic video action recognition tasks on the Kinetics400, UCF101 and HMDB51.
%
\ours achieves competitive results on fine-tuning experiments, indicating it can learn strong holistic visual representations in videos.
}
\label{tab:classification_table}
\vspace{-5pt}
\end{table}

==> ConST-CL (Arxiv-2)/Tex/Experiments/1.experiment_setup.tex <==
\subsection{Implementation Details}
\label{sec:implementation_details}
We use the ResNet3D-50 (R3D50) as our backbone feature extractor following~\cite{qian2021cvrl}.
All features are $\ell_2$ normalized before being used to compute the self-supervised loss.

For the holistic representation learning branch, we use a 3-layer MLP with $2048$ hidden nodes to project a $2048$-dimensional feature vector into a $128$-dimensional feature vector.
%
On the local representation learning branch, we use the same attention-based architecture as described in~\cite{vaswani2017attention}. 
%
The attention units are stacked into multiple heads and layers to construct the \ours head for the instance prediction task.
%
In this work, the head of \ours consists of 3-layer 3-head attention units with hidden dimension of $128$.
%
We use the ReLU activation function without dropout. 
%
A final linear layer is used to project the $128$-dim feature vector back to $2048$-dim.
%
We add spatio-temporal positional encodings to the query, key and value tokens before inputting into the transformer head in order to preserve location information. 
%
To construct contrastive pairs for local branch, we always sample examples from the center frame in both views for the experiments unless otherwise specified. 
%
The self-supervised pre-training is performed on the Kinetics400~\cite{kay2017k400} dataset.
%
During evaluations, all the heads used for self-supervised learning are discarded.

All models are pre-trained with mini-batch of $1024$. 
%
During the pre-training, we use the SGD optimizer with momentum of $0.9$.
%
The learning rate is linearly warmed-up to $40.96$ during the first $5$ epochs, followed by half-period cosine learning rate decay~\cite{he2019bag_of_tricks} to $0$. 
%
A weight decay of $10^{-6}$ is applied to all kernels.
%
We set the temperature $\tau$ to be $0.1$ for the global loss and $0.2$ for the local loss. 
%
The scale factor $\omega$ is $0.01$ to balance the global and local losses.

For results in Table (\ref{tab:main_table},\ref{tab:classification_table}), we pre-train the backbone model for $200$k steps, which is around $850$ epochs on the Kinetics400 dataset with the randomly generated region boxes. 
And the context length is set to $5$.
%
For all ablation studies, we use backbone models from a shorter pre-training schedule, which trains for $100$k steps.
% 
% The source code and trained models are planned to release to the public. 

==> ConST-CL (Arxiv-2)/Tex/Experiments/2.downstream_evaluations.tex <==
\subsection{Downstream Tasks}
% Most recent methods on video self-supervised learning focus on either improving the holistic representations or modeling local features.
%
%MH: colloquial
%We are naturally curious to ask whether those two domains can be combined together, as intuitively the better instance-level representations could be beneficial to the global recognition task and vice versa.
It is of great interest to understand whether one representation model can be applied to both holistic and local understandings, as intuitively the better local representations can facilitate holistic recognition tasks and vice versa.
%
In this work, we apply the learned representation models to (1) video action recognition tasks that require holistic representations on the  Kinetics400~\cite{kay2017k400}, UCF101~\cite{soomro2012ucf101} and HMDB51~\cite{kuehne2011hmdb} datastes; and (2) 
spatio-temporal action localization and single object tracking  tasks that require local representations on the  AVA-Kinetics~\cite{li2020avak}, AVA v2.2~\cite{gu2018ava} and OTB2015~\cite{wu2013otb} datasets. 

\noindent \textbf{Video action recognition.}
we perform linear evaluation by fixing all the backbone weights on Kinetics400~\cite{kay2017k400}, UCF101~\cite{soomro2012ucf101} and HMDB51~\cite{kuehne2011hmdb}. 
%
The input is a $32$-frame video clip with temporal stride of $2$ and resolution of $224$. We train the linear classifier for $100$ epochs.
%
% The feature vectors are $\ell_2$ normalized before feeding into the classifier.
%
% On UCF101~\cite{soomro2012ucf101} and HMDB51~\cite{kuehne2011hmdb}, 
We also use the pre-trained models to initialize the network and fine-tune all layers for $50$ epochs on UCF101 and HMDB51.

\noindent \textbf{Spatio-temporal action localization.} We attach the same action transformer head as in~\cite{girdhar2019vat,li2020avak} to our R3D50 backbone, and follow the setting in~\cite{li2020avak} for simplicity.
%
We train our model with ground-truth person bounding boxes and use either ground-truth boxes or boxes generated using off-the-shelf person detectors\footnote{We use the same set of boxes as in~\cite{li2020avak, feichtenhofer2021rho_moco} for fair comparisons.} for region proposals during evaluation. 
% \lzyuan{Rephrase: as the goal of these experiments is to evaluate the learned local feature representations rather than video detection.}
%
The model is trained with batch size $256$ for $50$k steps.
% , which is around $36$ epochs. 
%
The input has $32$ frames with resolution of $400$ and temporal stride of $2$.

\noindent \textbf{Single object tracking.} 
% Single object tracking is used for evaluating local representations as the high-quality semantically consistent features play an important role to determine object-level correspondence. 
We also evaluate our learned representations via single object tracking task, which requires semantically consistent spatio-temporal features to determine object-level correspondence.
%
We follow the same practice as in~\cite{xu2021vfs, gordon2020vince, yao2020seco} to adopt the SiameseFC~\cite{bertinetto2016siamese_fc} as the tracker and modify the spatial stride and dilation rate in the $res_4$ and $res_5$ blocks. 
%
Note that our backbone is a 3D-convolutional network, and for each input frame we also sample its neighboring $n$ frames from each side and use the $2n+1$ frames as the input. 
%
After the $res_5$ block, we slice the center frame along the time dimension of the local feature map $F$ for the input to the tracking head.
%
Here we use $n=2$ as the largest temporal kernel in the network is $5$.
%
We use the pre-trained checkpoint to initialize the backbone and fine-tune the tracker for all experiments.

==> ConST-CL (Arxiv-2)/Tex/Experiments/3.main_results.tex <==
\subsection{Main Results}
% lzyuan: Magic position, do not change!!!
% \input{Tables/temporal_sampling.tex}

%MH: check this sentence. Do not use "checkpoint" as it is colloquial and not everyone knows that it means.
In Table~\ref{tab:main_table}, we study the model performance on dense vision tasks by using the pre-trained models from different methods.
% \lzyuan{Justify the setting and rephrase: We evaluate the multi-instance action recognition on the AVA-Kinetics~\cite{li2020avak}.
% To reduce the complexity, we follow the common practice~\cite{li2020avak} to decouple the localization branch and show the action recognition performance.}
We evaluate the spatio-temporal action localization on the AVA-Kinetics~\cite{li2020avak} and AVA v2.2~\cite{gu2018ava}.
%
Following~\cite{li2020avak, girdhar2019vat}, the models are evaluated under two settings: using either ground-truth boxes or detected boxes as region proposals on the validation set.
%
On AVA-Kinetics, \ours achieves $39.4\%$ mAP when using ground-truth boxes and $30.5\%$ mAP when using detected boxes, outperforming the supervised method~\cite{li2020avak} by a large margin.
% It is interesting to note that \ours achieves more gains when using detected boxes($\Delta$) than using ground-truth boxes($\Delta 8.1$), comparing to the supervised training method.
% This indicates the better generalization ability of self-supervised training.
\ours also outperforms the baseline self-supervised method CVRL~\cite{qian2021cvrl} model 
with more than $24\%$ relative performance gain. 
%
In addition, we compare to the VFS~\cite{xu2021vfs} which is designed for dense vision tasks. 
%
As VFS uses 2D ResNet, we follow the common practice to inflate all 2D kernels in the network into 3D~\cite{carreira2017i3d} and load the pre-trained weights from VFS for the fair comparison.
%
In the table, \ours outperforms the VFS-inflated method by more than $4.6\%$ mAP, showing the effectiveness of our proposed method on spatio-temporal action recognition task.
%
On the AVA v2.2, we observe similar trend that \ours outperforms competing methods, achieving $31.1\%$ and $24.1\%$ mAP using ground-truth and detected boxes respectively.

% lzyuan: Magic position, do not change!!!
% \input{Tables/temporal_sampling.tex}
% \input{Tables/endpoints.tex}

%MH: redundant
%We chose single object tracking as another benchmark to testify the discriminativeness of the learned spatio-temporal representations, as the more discriminative an instance representation is across space and time, the easier the downstream tracker can learn to track the object in videos.
On OTB2015~\cite{wu2013otb}, we first compare with prior methods designed for dense task \textit{only}.
%
Table~\ref{tab:main_table} shows that 
\ours outperforms the evaluated methods by a large margin.
%
Specifically, compared to VFS~\cite{xu2021vfs}, \ours achieves $78.1\%$($+\Delta 4.2\%$) in precision score and $55.2\%$($+\Delta 2.7\%$) in success score.
%
To rule out the effect of architecture difference (2D network vs.\ 3D network), we inflate the 2D ResNet into 3D and load the VFS pre-trained checkpoint, denoted as VFS-inflated in the table.
%
Compared to VFS, VFS-inflated performs similarly to its 2D counterpart, which indicates the effect of this architecture difference on the tracking task is insignificant.
%
% Then we report model performance using CVRL pretrained model and note that CVRL outperforms VFS-inflated.
% Further, comparing to the CVRL pre-trained model, CVRL outperforms the VFS-inflated model.
% %
% Since the CVRL can be seen as the extension of VFS on clip-level pretraining, the improvement likely comes from a more homogeneous experiment setup.
%
When compared with CVRL, \ours achieves clear performance gain for single object tracking on the OTB2015 benchmark. 
%
% With the backbone model learned by \ours, our tracker achieves the state-of-the-art results in terms of precision and success scores on the OTB2015~\cite{wu2013otb} dataset.

In Table~\ref{tab:classification_table}, our method performs comparable to CVRL and $\rho$MOCO ($\rho$=2) using linear probing and achieves competitive fine-tuning results with top-1 accuracy of $94.8\%$ and $71.9\%$ on UCF101 and HMDB51, respectively. 
% 
It is worth pointing out that our method improves upon CVRL on fine-tuning UCF101 and HMDB51, even though we do not use any extra supervision on holistic representations other than the CVRL's loss $\mathcal{L}_g$. 
%
These findings are consistent with our intuition that the holistic and the local representation modeling can be mutually beneficial. 
% These findings are consistent with our intuition that holistic representation learning benefits from local self-supervision.
%
%MH: why do you say R4 here? Do you discuss R4 anywhere else before this?
In our method, the two losses simultaneously contribute to and constrain on the latent feature map $C4$ in the network. 
%
These results also demonstrate the effectiveness of the proposed model design that coherently organizes different levels of representations in a single framework.
% 

% lzyuan: Magic position, do not change!!!
% \input{Tables/context_length_and_overhead.tex}
% \input{Tables/box_type.tex}

Finally, in Table~\ref{tab:model_size} we report the model size and computational cost including \textit{both} the backbone and the SSL heads in different video self-supervised learning methods. 
% 
Comparing to CVRL, \ours increased model sizes and computational cost moderately, mainly due to the branched $res_5$ block and additional transformer head.
% 
The Slow-only network and training strategy used in~\cite{feichtenhofer2021rho_moco} is different from ours, making the side-to-side comparison difficult. 
% 
Thus we leave the results in the table for reference. 

==> ConST-CL (Arxiv-2)/Tex/Experiments/4.ablation_studies.tex <==
\subsection{Ablation Study}
% \input{Tables/context_length_and_overhead.tex}

\label{sec:ablations}
% In this section, we conduct ablation studies to analyze how several key designs affect the spatio-temporal representation learning using \ours.

\noindent \textbf{Temporal sampling strategy.}
% \input{Tables/temporal_sampling.tex}
% In the model described in Section~\ref{sec:contextualization}, we do not constrain the number of regions drawn from the source view and the temporal locations they should be transformed into in the target view.
% %
% For computational and memory efficiency, we sample one frame from the source and one frame from the target view, and then sample regions to construct the pairs.
%
To construct the contrastive region pairs, we sample one frame from the source and the target clip respectively.
%
In Table~\ref{tab:sampling}, we study three different temporal sampling strategies.
%
For ``random" strategy, we randomly sample frames from the source and the target views to construct the contrastive pairs.
%
For ``center" strategy, we simply choose the center frame from the dense feature maps in both views for  \ours.
%
For ``nearest" strategy, we always choose the temporally closest frame pairs from two views. 
%
If two randomly sampled clips temporally overlap, then we draw samples from their overlapping frames.
%
Otherwise, frames at the closest two ends of the two video clips are selected.
%
Table~\ref{tab:sampling} shows that the ``random" sampling strategy is consistently worse than the other approaches.
%
This can be attributed to that the temporally random sampling introduces significant noise and negatively affect the model performance.  
%
%MH: do not use don't, didn't, just write out the whole words
%We didn't observe significant difference between ``Center" and ``Nearest" strategy. 
We do not see significant performance differences by using the ``center" or ``nearest" sampling strategy. 
%
For the simplicity, we choose the ``center" sampling strategy throughout our experiments.

%MH: is endpoint a typical term to analyze loss function in network model? 
%MH: I do not know the technical details of this section. So, you need to read it carefully and ask others to proofread it
\noindent \textbf{Loss endpoints.}
% \input{Tables/endpoints.tex}
% \input{Tables/context_length_and_overhead.tex}
%We believe that global and local contrastive losses could contribute to each other if we combine them in an organic way. 
We analyze how global and local contrastive losses can be integrated together for vision tasks. 
%
In this study, we attach the proposed local loss to different endpoints of the network and analyze how it interacts with the global loss.
%
As shown in Fig.~\ref{fig:global_local_loss}(a) the region features are from the C5 endpoint for this model. 
%
For the model in Fig.~\ref{fig:global_local_loss}(b), we first perform a 2$\times$2 average pooling on the C4 feature map to reduce its spatial resolution from 14$\times$14 to 7$\times$7 and then apply the region-level loss.
%
For the model in Fig~\ref{fig:global_local_loss}(c), we duplicates the $res5$ block of the network and then apply the global loss on $\text{C5}_g$ branch and the region loss on the $\text{C5}_r$ branch respectively.
%
During the inference stage for the model in Fig~\ref{fig:global_local_loss}(c), we use feature maps from $\text{C5}_g$ and $\text{C5}_r$ for video and instance-level tasks respectively.
%
In Table~\ref{tab:endpoints}, we observe that by simply adding the proposed region-based contrastive loss on C4$_p$ or C5, \ours outperforms the baseline method CVRL on downstream tasks already.
% Empirically the self-supervised learning using configuration (a) or (b) is prone to hyperparameter tuning to balance the effect of two losses. 
By branching the $res5$ block as shown in Fig~\ref{fig:global_local_loss}(c), we achieve the best trade-off of two losses and the holistic and local representations obtain better performance gains on downstream tasks.

\noindent \textbf{Context length.}
% \input{Tables/context_length.tex}
% \input{Tables/context_length_and_overhead.tex}
We study the effect of contextualization by varying the number of feature maps sampled along the time axis from the target view to input to the \ours transformer head.
%
Different number of context length indicates the number of feature maps sampled along the time axis.
%
Note that when the context length is zero, the method simply degrades to the vanilla region-based contrastive learning described in Section~\ref{sec:icl}. 
%
Table~\ref{tab:context_length_and_overhead} shows 
our model learns better representations as the context length is increased. 
%
This can be attributed to that as more context features provide richer information about the target view, the model can learn a better decoder function $g(\cdot, \cdot)$, resulting in higher-quality spatio-temporal representations.
% \noindent \textbf{Computational overhead.} 
% \input{Tables/computational_cost}
%One may be curious about the computational overhead with different types of self-supervised training configurations.
%
In Table~\ref{tab:context_length_and_overhead}, we also present the number of model parameters and FLOPs for one pass of self-supervised training.
% $0$ context length means we use the MLP head to project the region features instead of the transformer head, in which case our pretraining degraded to the vanilla region based contrastive learning as described in Section~\ref{sec:icl}.
Comparing the vanilla region-based model (second row) to the baseline model CVRL (first row), we note that the number of model parameters is increased by $74.2\%$ and the number of FLOPs is increased by $20.9\%$, where the overheads largely result from the duplicated $res5$ block.
%
When switching to the proposed transformer decoder with context length equals to $1$, the number of model parameters is decreased to $71.76$M while the FLOPs is increased by $0.16$B.
%
This is due to the fact that we use multi-head self-attention with fewer hidden units, which is more parameter efficient.
%
Finally, when increasing context lengths, we notice only slight increases in the number of FLOPs.

\noindent \textbf{Boxes type.}
% \input{Tables/box_type.tex}
Table~\ref{tab:box_type} shows how different location priors affect the representations learning.
% In the study, we found that regardless of the region location's quality, the model learns equally-well representations and across the downstream tasks
%MH: bottom rows? (two detectors)?
%In the table, the lower row uses boxes that are supposed to be more accurate and general.
We study three types of boxes generated using different methods: randomly generated boxes, boxes derived from low-level image cues and detector-generated boxes. 
%
Overall, our method performs equally well regardless whether region locations are accurate or not.
% \liuti{The insight below is superficial, needs rewriting.}
% Overall, different box types have insigificant performance differences.
%
We reason that each region could be understood as an instance crop in the scene and \ours does not require the crop to be object-centric.
% the model learns to produce temporally persistent but discriminative features during the self-supervised training.
This observation is aligned with previous self-supervised learning methods on images~\cite{he2019moco, chen2020simclr} and videos~\cite{qian2021cvrl}.
The experiment suggests the robustness of the proposed method.
% \lzyuan{(MH: I do not quite understand the logic in the following three sentences (i.e., I do not quite agree with the explanations). Ask others to proofread them.) TODO}
% Due to scene consistency in a video, randomly generated boxes in different frames likely have overlaps on the same instances.
% %
% Then these two regions share the scene semantics overlap across space and time serve as the positive examples during the training.
% %
% This mechanism is similar to the aggressive spatial augmentation commonly adopted for the self-supervised learning models for images, except that the correspondences are learned in our case.


==> ConST-CL (Arxiv-2)/Tex/Method/1.instance_constrastive_learning.tex <==
\subsection{Region-Based Contrastive Learning in Videos}
\label{sec:icl}
% Given an image sequence, a simple contrastive learning pipeline for video representation first samples two segments $\{x, x^\prime\}$ randomly.
%
% Temporally consistent data augmentations, including random cropping, flipping, color jittering and blurring, are then applied independently on each clip.
%
% The video-level representations $\{z, z^{\prime}\}$ in $\mathbb{R}^c$, extracted by the feature extractor, are regularized by the InfoNCE loss~\cite{oord2018info_nce}.
Given a video, a simple contrastive learning algorithm randomly samples two video clips $\{x, x^\prime\}$, and applies random data augmentation on each video clip independently.
Corresponding video-level representations $\{z, z^{\prime}\}\in\mathbb{R}^C$ are extracted by the network $f(\cdot)$ for computing a contrastive loss~\cite{oord2018info_nce}, with negative examples from other videos.
%
We denote this video-level global contrastive loss as $\mathcal{L}_g$.
%
This training objective enforces globally average-pooled features from the same video to be similar while it repels such features from different videos.
%
However, no explicit supervision is enforced on local features, which play an important role for dense prediction tasks.

% Recent self-supervised learning methods~\cite{wang2021densecl,henaff2021cont_det,xie2021propagate} apply the InfoNCE~\cite{oord2018info_nce} loss on the dense feature map before the average pooling layer, and perform well on dense prediction tasks.
%
% One straightforward extension is to apply 
% a similar approach as~\cite{wang2021densecl} for spatio-temporal representation learning in videos.  
To enforce local supervision, one way is to extend~\cite{wang2021densecl} to the spatio-temporal domain.
%
Given the dense feature maps $\{F, F^{\prime}\}\in\mathbb{R}^{T \times H \times W \times C}$ from $\{x,x^{\prime}\}$, where $T, W, H, C$ are time, height, width and channel dimention respectively, for each feature voxel $h_i \in F$, we find its correspondence $h_j^{\prime} \in F^{\prime}$ that it is closest to in the feature space to form a positive pair.
%
% More details on how to find the dense correspondence can be found in~\cite{wang2021densecl}. 
%
Thus, the dense contrastive loss in a video can be formulated as:
\begin{align}
    z_i &= g(h_i) = \text{MLP}(h_i),\label{eq:dense_cl_z} \\
    \mathcal{L}_{r} &= \sum_i -\log \frac{\exp(z_i \cdot z_j^{\prime}/\tau)}{\exp(z_i \cdot z_j^{\prime}/\tau) + \sum_k {\exp(z_i \cdot \hat{z}_k/\tau)}}, \notag \\
    \mbox{s.t.} &\quad j = \argmin_j h_i \cdot h^\prime_j,\label{eq:dense_cl_loss}
\end{align}
where MLP refers to a multi-layer perceptron, $\tau$ is the temperature parameter, $i$, $j$ and $k$ are grid indices, and $\{\hat{z}\}$ are representations from other videos.
%
Here, we simply regard all the dense features from other videos as negative examples for loss computation. 
% \lzyuan{Rephrase: However, one obvious drawback of such dense contrastive learning method is that the feature maps are artificially discretized into grid and the cross-boundary objects are cut into pieces.
% This may lead to inferior representation quality and the training in-stability due to the discretization and ambiguous correspondence.}

Assuming that we have access to the location priors of regions of interest $\{r_i\}$, we can derive the vanilla region-based contrastive learning by organizing the representations using the region location:
% Further, given a set of instance regions $\{r_i\}$, we can derive a vanilla instance-based local contrastive loss following Eq.~(\ref{eq:dense_cl_loss}) by replacing Eq.~(\ref{eq:dense_cl_z}) with
\begin{align}
    z_i &= g(h_i) = \text{MLP}(\text{ROIAlign}(F, r_i)),\label{eq:unary_region_z}
    % \mathcal{L}_r &= -log \frac{exp(z_i \cdot z_j^{\prime}/\tau)}{exp(z_i \cdot z_j^{\prime}/\tau) + \sum_{n=1}^N {exp(z_i \cdot \hat{z_n}/\tau)}}
    % \label{eq:inst_loss}
\end{align}
where we override the notation $h_i$ to be the pooled region features, with $i$ being the region index. 
In this paper, we parameterize a region as a bounding box of a certain frame $r = \{t, x_{\textrm{min}}, y_{\textrm{min}}, x_{\textrm{max}}, y_{\textrm{max}}\}$. 
The region representation $h_i$ is pooled from the dense feature map $F$ by ROIAlign~\cite{ren2015faster-rcnn}. 

The full learning objective is the linear combination of the global loss and the local loss weighted by the scale factor $\omega$. And we average over the $N$ mini-batch during training: 
\begin{align}
    \mathcal{L} = \frac{1}{N} \sum \left(\mathcal{L}_g + \omega \mathcal{L}_r\right).
\end{align}
% In the following, we will discuss how to generate boxes in the next section and study the effect of box accuracy on qualify of the learned representations.

==> ConST-CL (Arxiv-2)/Tex/Method/2.contextualized_instance_prediction.tex <==
\subsection{Contextualized Spatio-Temporal Contrastive Learning (\ours)}
\label{sec:contextualization}
The vanilla region-based contrastive learning framework described in Section~\ref{sec:icl} has one limitation: the loss always encourages the representations of the same instance at different timestamps to be similar, 
while the appearance of an instance in a video may change across frames.
% \lzyuan{Visual dynamics sounds like a property of a representation, while we may want to high-light the difference between two representations?} which fails to capture visual dynamics in videos.
%
For example, one person in a video can appear in different poses and perform different activities.
%
Simply enforcing the similarity of the same instance at different temporal locations of the video will inadvertently encourage the model to encode only the minimal information, which is less effective for downstream video understanding tasks. 

% Based on this observation, 
To resolve this issue, we propose a novel self-supervised method, Contextualized Spatio-Temporal Contrastive Learning (\ours).
% , that learns to encode spatio-temporally fine-grained representations during the pre-training process.
In a nutshell, \ours requires the network to learn to ``reconstruct" the representation of a region in a target view given its representation from the source view and the context features around the target view.
\begin{align}
    z_i &= g(h_i, F_c^\prime) = g(\text{ROIAlign}(F, r_i), F_c^\prime),\label{eq:binary_region_z} \\
    \mathcal{L}_r &= \sum_i -\log \frac{\exp(z_i \cdot h_j^{\prime}/\tau)}{\exp(z_i \cdot h_j^{\prime}/\tau) + \sum_k {\exp(z_i \cdot \hat{h}_k/\tau)}}, \notag \\
    \mbox{s.t.} &\quad j = \argmin_j h_i \cdot h^\prime_j,\label{eq:inst_loss}
\end{align}
where $F^{\prime}_c$ denotes the set of context features around the target view, and $i$, $j$ and $k$ are region indices, and $\{\hat{h}\}$ are representations from other videos.
Here we would like to note: (1) comparing with Eq.~(\ref{eq:unary_region_z}), we extend the representation decoding function $g(\cdot)$ from an unary function to a binary function $g(\cdot,\cdot)$ in Eq.~(\ref{eq:binary_region_z});
% , which we will introduce in details later in this section; 
(2) we do not force bijective mapping between regions in two clips, so the different numbers of regions between views do not cause a problem.
% (2) the asymmetric formulation for the similarity computation in Eq.~(\ref{eq:inst_loss}). 
Eq.(\ref{eq:binary_region_z}-~\ref{eq:inst_loss}) formulate ConST-CL in a general manner, which considers all regions from all frames. 
It might pose computation challenges, so in practice, we instead construct two sets of regions by sampling from one temporal slice of each feature map. 
The temporal sampling strategy will be discussed in the following ablation studies.

Fig.~\ref{fig:method} shows an illustration of \ours. 
Given a pooled region feature $h_i$ from the source view and a set of context features $F^\prime_c$ from the target view, a projection function $z_i = g(h_i, F^\prime_c)$ is learned with the objective to minimize the representation distance between the reconstructed relating representation $z_i$ and its corresponding native representation $h_j^\prime$ in the target view.
%
The context features $F^\prime_c$ are a subset of feature voxels sampled from the dense feature map $F^\prime$.
In our case, we subsample a few frames from the dense video representations $F^\prime$ along the temporal dimension.
%
We define the number of frames used to construct $F^\prime_c$ as the \textit{context length}, whose effect on the performance is studied in Section~\ref{sec:ablations}.
%
Different from simply contrasting features that are projected into the shared feature space, \ours requires every feature vector in $\{F, F^\prime\}$ to encode more information about itself and the context, such that with context features from another view, $g(\cdot, \cdot)$ can reconstruct the instance encoding conditionally.

% In this work, we use the transformer~\cite{vaswani2017attention} architecture as the decoding function $g(\cdot, \cdot)$. 
We implement $g(\cdot,\cdot)$ using a transformer~\cite{vaswani2017attention} architecture.
%
First, we linearly project each instance feature vector from the source view $h_i$ to a Query token, and the context feature vectors from the target view $F_c^\prime$ to Key-Value token pairs. 
%
The multi-head cross-attention is then used to look up the Key-Value pairs by the Query token.
% \liuti{Add one or two sentences here about intuitively what this transformer head does, and why it is good for alleviating the aforementioned issue.}
% and the input Query token is transformed to the target domain. %
Finally, we apply the InfoNCE loss~\cite{oord2018info_nce} on the transformed instance feature $z_i$ and its correspondence $h_j^\prime$ using Eq.~(\ref{eq:inst_loss}).

==> ConST-CL (Arxiv-2)/Tex/Method/3.instance_locations.tex <==
\subsection{Region Generation}
\label{sec:box_generation}
% We conduct numerous experiments to analyze the effect of location prior on self-supervised representation learning. 
% We study the region locations generated from different sources.
% In this section, we introduce three options to generate region priors that we study for training \ours. 
% Note that the hyperparameters mentioned in this section are fixed for all the related experiments in this paper.

\noindent \textbf{Random boxes.} Generating random boxes on-the-fly during the training is the most straightforward method. 
%
For all of our related experiments, we randomly generate $8$ boxes on each frame. 
%
% The boxes are constrained to have aspect ratio within $[0.5, 2]$ and size within $[0.1, 0.5]$ of the image size.
%
% Interestingly, our method performs robustly whether the boxes are generated accurately or not (see Section~\ref{sec:ablations}).
In Section~\ref{sec:ablations}, we show that our method performs interestingly well trained with these random boxes.

% \textbf{Boxes from computational image masks.} 
\noindent \textbf{Boxes from low-level image cues.}
We also consider two methods to generate boxes from low-level image cues. 
%
Specifically, we use the SLIC~\cite{achanta2012slic} algorithm to generate $16$ superpixels on each frame. 
%
Following~\cite{henaff2021cont_det}, we alternatively use the graph-based image segmentation method~\cite{felzenszwalb2004fh_seg} to generate $16$ image segments for each frame. 
%
% We use two scales to generate segments, the scale $s$ and minimum cluster size $c$, and $s=c \in \{500, 1000\}$ in practice.
% We use two sets of (scale, minimum cluster size), i.e., $(500,500)$ and $(1000,1000)$, in practice to generate segments.
%
% After the segments generation, we convert each segment into its minimal bounding box and only keep those with width/height between $[0.05, 0.7]$ of the image width/height.

\noindent \textbf{Boxes from detectors.} 
We also use off-the-shelf modern detectors to generate object-centric bounding boxes for weakly supervised learning.
%
A CenterNet-based~\cite{zhou2019centernet} person detector is employed to generate bounding boxes on persons only. 
%
%The detector is trained on the COCO person detection dataset~\cite{lin2014coco_dataset}.
%
As an alternative, we use a generic object detector, which is based on Cascade RCNN~\cite{du2021crcnn}. 
%and is trained on COCO object detection dataset~\cite{lin2014coco_dataset}.

% It is worth pointing out human supervision is essentially used using detector-generated boxes for training \ours. For all of our experiments, we use random boxes, except in the box type ablation study (Section~\ref{sec:ablations}) we compare the performances using these three types of boxes.


==> ConST-CL (Arxiv-2)/Tex/Method/3.instance_locations_bk.tex <==
\subsection{Region Generation}
\label{sec:box_generation}
% We conduct numerous experiments to analyze the effect of location prior on self-supervised representation learning. 
% We study the region locations generated from different sources.
In this section, we introduce three options to generate region priors that we study for training \ours. 
% Note that the hyperparameters mentioned in this section are fixed for all the related experiments in this paper.

\noindent \textbf{Random boxes.} Generating random boxes on-the-fly during the training is the most straightforward method. 
%
For all of our related experiments, we randomly generate $8$ boxes on each frame. 
%
The boxes are constrained to have aspect ratio within $[0.5, 2]$ and size within $[0.1, 0.5]$ of the image size.
%
% Interestingly, our method performs robustly whether the boxes are generated accurately or not (see Section~\ref{sec:ablations}).
In Section~\ref{sec:ablations}, we show that our method performs interestingly well trained with these random boxes.

% \textbf{Boxes from computational image masks.} 
\noindent \textbf{Boxes from low-level image cues.}
We also consider two methods to generate boxes from low-level image cues. 
%
Specifically, we use the SLIC~\cite{achanta2012slic} algorithm to generate $16$ superpixels on each frame. 
%
Following~\cite{henaff2021cont_det}, we alternatively use the graph-based image segmentation method~\cite{felzenszwalb2004fh_seg} to generate $16$ image segments for each frame. 
%
We use two scales to generate segments, the scale $s$ and minimum cluster size $c$, and $s=c \in \{500, 1000\}$ in practice.
% We use two sets of (scale, minimum cluster size), i.e., $(500,500)$ and $(1000,1000)$, in practice to generate segments.
%
After the segments generation, we convert each segment into its minimal bounding box and only keep those with width/height between $[0.05, 0.7]$ of the image width/height.

\noindent \textbf{Boxes from detectors.} 
We also use off-the-shelf modern detectors to generate object-centric bounding boxes for weakly supervised learning.
%
A CenterNet-based~\cite{zhou2019centernet} person detector is employed to generate bounding boxes on persons only. 
%
%The detector is trained on the COCO person detection dataset~\cite{lin2014coco_dataset}.
%
As an alternative, we use a generic object detector, which is based on Cascade RCNN~\cite{du2021crcnn}. 
%and is trained on COCO object detection dataset~\cite{lin2014coco_dataset}.

% It is worth pointing out human supervision is essentially used using detector-generated boxes for training \ours. For all of our experiments, we use random boxes, except in the box type ablation study (Section~\ref{sec:ablations}) we compare the performances using these three types of boxes.


==> ConST-CL (Arxiv-2)/Tex/Method/4.balance_global_local.tex <==
\subsection{Balancing Global and Local Losses}
Existing methods~\cite{zhou2016cams, xu2021vfs} have shown discriminative local features can be extracted 
by applying supervisory signals on holistic representations. 
%
Intuitively, adding constraints on both holistic and local representations are mutually beneficial, because discriminative local features would contribute to holistic recognition, while expressive holistic features could be derived from local features.
%
In practice, however, we find that directly adding the proposed region-based local loss on the dense feature map right before the average pooling layer in the ResNet, the self-supervised training is less stable and sensitive to the hyper-parameters for balancing the global and local losses. 

To address this issue, we propose a simple solution. 
%
As we use ResNet3D-50 as our base model, instead of adding the local loss on the $C5$ endpoint, we modify the ResNet architecture and replicate the $res5$ block, forming a ``Y'' structure, as shown in Fig.~\ref{fig:global_local_loss}.
%
Then the global and local losses are attached on endpoint $C5_g$ and $C5_r$, respectively, and they co-constrain the latent feature map in $C4$ during training.
%
When fine-tuning the model for downstream tasks, we take either $C5_g$ or $C5_r$ branch depending on the task.
%
This design introduces only moderate additional computes during the pre-training stage and is at no extra cost for fine-tuning and inference. 
%
We will show in Section~\ref{sec:ablations} that the proposed ``Y'' structure results in better trade-off for both video-level and instance-level downstream tasks.

==> Tables/computational_cost.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{cccc} 

\hline
Context length & Endpoint & $\#$ Params (M) & FLOPs (B) \\
\hline
- & - & $44.60$ & $45.58$ \\
% $0$ & R5 & $57.48$ & $45.68$ \\
$0$ & 2R5 & $77.71$ & $55.45$ \\
$1$ & 2R5 & $71.76$ & $55.60$ \\
% $3$ & 2R5 & $71.76$ & $56.07$ \\
$5$ & 2R5 & $71.76$ & $56.53$ \\
\hline

\end{tabular}
\caption{
Ablation study on the computational cost. 
We notice the number of parameter increment is largely from the duplicated $res5$ block while our transformer based head is more parameter efficient than the MLP head for the region-based contrastive learning.
}
\label{tab:cost}
\end{table}

==> Tables/context_length.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{cccccc} 

\hline
Context &  \multicolumn{2}{c}{AVA-Kinetics} & &  \multicolumn{2}{c}{OTB}\\
\cline{2-3} \cline{5-6}
length & mAP (GT) & mAP (Det) & & Precision & Success\\
\hline
 - & $30.9$ & $23.4$ & & $75.9$ & $53.6$ \\
$0$ & $35.3$ & $27.5$ & & $75.4$ & $56.6$ \\
$1$ & $36.7$ & $28.0$ & & $77.7$ & $55.0$ \\
$3$ & $36.9$ & $28.1$ & & $77.5$ & $54.5$ \\
$5$ & $37.6$ & $28.1$ & & $79.0$ & $55.4$ \\
\hline

\end{tabular}
\caption{
We analyze the effect of context length to the model performance. 
``-" indicates no \ours is used and the model is only trained with the $\mathcal{L}_g$; 
``0" indicates no context is provided and the model simply degraded to the vanilla region-based contrastive learning.
From the table, we observe the trend that more context is helpful to learn better spatio-temporal representations.}
\label{tab:context_length}
\end{table}

==> Tables/main_table_bk.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{cccccccccccccccc} 
\hline
 
 &  & Pre-training & Linear & \multicolumn{2}{c}{Fine-tune} & & \multicolumn{2}{c}{Action Localization} & &  \multicolumn{2}{c}{Object Tracking} \\
\cline{5-6} \cline{8-9} \cline{11-12}
Method & Backbone & Dataset & K400 & UCF & HMDB & & AVA-K (GT) & AVA-K (Det) & & Precision & Success \\

\hline
INet-sup~\cite{li2020avak} & I3D & K400 & - & - & - & & $35.9$ & $22.9$ & & - & -\\
INet-sup$^{\dagger}$ & I3D & K400 & - & - & - & & $32.0$ & $23.1$ & & - & -\\
K400-sup & R3D50 & K400 & - & - & - & & $26.7$ & $19.8$ & & $71.2$ & $51.46$ \\
\hline
SimSiam~\cite{chen2021simsiam} & R50 & INet & - & - & - & & - & - & & $61.0$ &  $43.2$ \\
VINCE~\cite{gordon2020vince} & R50 & R2V2 & $49.1$ & - & - & & - & - & & $66.0$ & $47.6$ \\
SeCo~\cite{yao2020seco} & R50 & K400 & $61.9$ & $88.3$ & $55.6$ & & - & - & & $71.9$ &  $51.8$ \\
VFS~\cite{xu2021vfs} & R50 & K400 & - & - & - & & - & - & & $73.9$ &  $52.5$ \\
\hline
$\rho$MoCo~\cite{feichtenhofer2021rho_moco} & R3D50 & K400 & $\mathbf{67.4}$ & $93.2$ & - & & - & - & & - & - \\
VFS-inflated & R3D50 & K400 & $33.1$ & $71.4$ & $41.0$ & & $34.6$ & $25.9$ & & $73.3$ & $52.7$ \\
CVRL~\cite{qian2021cvrl} & R3D50 & K400 & $66.1$ & $92.2$ & $66.7$ & & $31.6$ & $24.1$ & & $75.4$ & $53.7$ \\
\hline
\ours & R3D50 & K400 & $66.6$ & $\mathbf{94.8}$ & $\mathbf{71.9}$ & & $\mathbf{39.4}$ & $\mathbf{30.5}$ & & $\mathbf{78.1}$ & $\mathbf{55.2}$ & \\

\hline

\end{tabular}
% \caption{We evaluate the self-supervised learning in two folds: the fine-grained spatio-temporal understanding on AVA-Kinetics and OTB and the holistic video understanding on K400, UCF101 and HMDB51.
\caption{\textbf{Downstream task performances using pre-trained representations.} The learned representations are evaluated for spatio-temporally fine-grained tasks, including spatio-temporal action recognition on AVA-Kinetics (using both ground-truth and detected person boxes) and single object tracking on OTB2015, and holistic video action recognition tasks on Kinetics400, UCF101 and HMDB51.
%
\ours achieves the state-of-the-art results across the board, suggesting the effectiveness of our proposed framework that is capable of coherently learning better holistic and local visual representations in videos.
$^{\dagger}$ indicates our reproduced results.}
\label{tab:main_table}
\vspace{-10pt}
\end{table*}

==> Tex/Method/3.instance_locations_bk.tex <==
\subsection{Region Generation}
\label{sec:box_generation}
% We conduct numerous experiments to analyze the effect of location prior on self-supervised representation learning. 
% We study the region locations generated from different sources.
In this section, we introduce three options to generate region priors that we study for training \ours. 
% Note that the hyperparameters mentioned in this section are fixed for all the related experiments in this paper.

\noindent \textbf{Random boxes.} Generating random boxes on-the-fly during the training is the most straightforward method. 
%
For all of our related experiments, we randomly generate $8$ boxes on each frame. 
%
The boxes are constrained to have aspect ratio within $[0.5, 2]$ and size within $[0.1, 0.5]$ of the image size.
%
% Interestingly, our method performs robustly whether the boxes are generated accurately or not (see Section~\ref{sec:ablations}).
In Section~\ref{sec:ablations}, we show that our method performs interestingly well trained with these random boxes.

% \textbf{Boxes from computational image masks.} 
\noindent \textbf{Boxes from low-level image cues.}
We also consider two methods to generate boxes from low-level image cues. 
%
Specifically, we use the SLIC~\cite{achanta2012slic} algorithm to generate $16$ superpixels on each frame. 
%
Following~\cite{henaff2021cont_det}, we alternatively use the graph-based image segmentation method~\cite{felzenszwalb2004fh_seg} to generate $16$ image segments for each frame. 
%
We use two scales to generate segments, the scale $s$ and minimum cluster size $c$, and $s=c \in \{500, 1000\}$ in practice.
% We use two sets of (scale, minimum cluster size), i.e., $(500,500)$ and $(1000,1000)$, in practice to generate segments.
%
After the segments generation, we convert each segment into its minimal bounding box and only keep those with width/height between $[0.05, 0.7]$ of the image width/height.

\noindent \textbf{Boxes from detectors.} 
We also use off-the-shelf modern detectors to generate object-centric bounding boxes for weakly supervised learning.
%
A CenterNet-based~\cite{zhou2019centernet} person detector is employed to generate bounding boxes on persons only. 
%
%The detector is trained on the COCO person detection dataset~\cite{lin2014coco_dataset}.
%
As an alternative, we use a generic object detector, which is based on Cascade RCNN~\cite{du2021crcnn}. 
%and is trained on COCO object detection dataset~\cite{lin2014coco_dataset}.

% It is worth pointing out human supervision is essentially used using detector-generated boxes for training \ours. For all of our experiments, we use random boxes, except in the box type ablation study (Section~\ref{sec:ablations}) we compare the performances using these three types of boxes.

